Dependence-Aware, Unbounded Sound Predictive Race Detection

Data races are a real problem for parallel software, yet hard to detect. Sound predictive analysis observes a program execution and detects data races that exist in some other, unobserved execution. However, existing predictive analyses miss races because they do not scale to full program executions or do not precisely incorporate data and control dependence. This paper introduces two novel, sound predictive approaches that incorporate data and control dependence and handle full program executions. An evaluation using real, large Java programs shows that these approaches detect more data races than the closest related approaches, thus advancing the state of the art in sound predictive race detection.

==> BR-only-no-branch.tex <==
%auto-ignore
\begin{figure}

\small
\centering

\subfloat[\WCP analysis misses the predictable race]{
\centering
\sf
\makebox[.4\linewidth]{
\begin{tabular}{@{}ll@{}}
\textnormal{Thread 1} & \textnormal{Thread 2} \\\hline 
wr(y)                 & \\
acq(m)                & \\
wr(x)                 & \\
rel(m)\tikzmark{1}    & \\
                      & acq(m) \\
                      & \tikzmark{2}rd(x) \\
                      & rel(m) \\
                      & wr(y) \\
                      & \\
\end{tabular}}
\label{fig:BR-only:no-branch:race}}
\subfloat[No predictable race exists]{
\centering
\sf
\makebox[.4\linewidth]{
\begin{tabular}{@{}ll@{}}
\textnormal{Thread 1} & \textnormal{Thread 2} \\\hline 
wr(y)                 & \\
acq(m)                & \\
wr(x)                 & \\
rel(m)\tikzmark{3}    & \\
                      & acq(m) \\
                      & \tikzmark{4}rd(x) \\
                      & \tikzmark{5}\BrUniv \\
                      & rel(m) \\
                      & wr(y)
\end{tabular}}
\label{fig:BR-only:no-branch:no-race}}

\textlink{1}{2}{\DC}
\textlink{3}{4}{\DC}
\textunderlink{3}{5}{\WBR}

\mike{This figure overlaps with Figure~\ref{fig:simple-BR} quite a bit. Remove this figure?}

\caption{There is a predictable race on \texttt{y} in (a), but not in (b). Note
  that in (a) there is no branch event after the read on x in Thread 2: If the
  critical sections in Thread 2 executed first, even though the read of x
  observes a different value, the execution would continue without any change at
  least until the write to y. \DC (and thus \WCP) miss the race in (a); \BR (and thus \WBR) are able
  to report it.}
\end{figure}


==> BR-soundness-proof.tex <==
%auto-ignore
\section{\BR Soundness Proof}
\label{sec:br-soundness-proof}

\mike{The following is a start at another way to prove \BR soundness.}

\begin{proof}[Alternate \BR soundness proof]
Let \tr be an execution trace whose first \BR-race is between events \event{e}{_1} and \event{e}{_2},
where \emph{first} means that \event{e}{_2} is as early as possible in \tr and among \BR-races whose second event is \event{e}{_2},
\event{e}{_1} is as late as possible in \tr.
Suppose \tr has no predictable race or deadlock.
Thus \tr has no \emph{\WCP-race}, since \WCP is sound~\cite{wcp}.

Then \TROrdered{\event{e}{_1}}{\event{e}{_2}},
\conflicts{\event{e}{_1}}{\event{e}{_2}},
\WCPOrdered{\event{e}{_1}}{\event{e}{_2}},
\nBROrdered{\event{e}{_1}}{\event{e}{_2}}, and
$\commonLocks{\event{e}{_1}}{\event{e}{_2}} = \emptyset$.

\event{e}{_1} and \event{e}{_2} can only be directly ordered by \WCP \Rule{\ref{wcp:hb-composition}}.
Maybe it makes sense to first prove something about any \WCP-ordered events (not just \event{e}{_1} and \event{e}{_2})?
% If \event{e}{_1} and \event{e}{_2} are ordered by \WCP \Rule{\ref{wcp:rule-a}},
% then $\commonLocks{\event{e}{_1}}{\event{e}{_2}} \ne \emptyset$, a contradiction.
% 
% If \event{e}{_1} and \event{e}{_2} are ordered by \WCP \Rule{\ref{wcp:rule-b}},
% then 
Use induction on \WCP-distance?

Or another way is to consider each case where \BR is weaker than \WCP,
like the following, but how to be rigorous about that?

\event{e}{_1} and \event{e}{_2} must be \WCP ordered but not \BR ordered because of some difference between
the relations. Consider if the difference is the handling of write--read conflicts.
Cannot be on \event{e}{_1} and \event{e}{_2} directly, since then $\commonLocks{\event{e}{_1}}{\event{e}{_2}} \ne \emptyset$, a contradiction.
Let \event{w}{} and \event{r}{} be write and read events, respectively, that are conflicting (\conflicts{\event{w}{}}{\event{r}{}}).

\end{proof}

% \begin{empty}
% 
% \newcommand{\OrderedT}[3]{\textcolor{red}{\ensuremath{#1 #2 #3}}}
% 
% \renewcommand{\nHBOrdered}[2]{\OrderedT{#1}{\nltHB}{#2}}
% \renewcommand{\HBOrdered}[2]{\OrderedT{#1}{\ltHB}{#2}}
% 
% \renewcommand{\BROrdered}[2]{\OrderedT{#1}{\ltBR}{#2}}
% \renewcommand{\EqBROrdered}[2]{\OrderedT{#1}{\ltEqBR}{#2}}
% \renewcommand{\nBROrdered}[2]{\OrderedT{#1}{\nltBR}{#2}}
% 
The following proof logic is inspired by prior work's proofs~\cite{causally-precedes,wcp}. 

\begin{thm}[\BR Soundness]
  If an execution trace \tr has a \BR-race,
  then \tr has a predictable race or a predictable deadlock.
\end{thm}

\begin{proof}
Let \tr be an execution trace whose first \BR-race is between events \event{e}{_1} and \event{e}{_2},
where \emph{first} means that \event{e}{_2} is as early as possible in \tr and among \BR-races whose second event is \event{e}{_2},
\event{e}{_1} is as late as possible in \tr.
% Then \TROrdered{\event{e}{_1}}{\event{e}{_2}},
% \conflicts{\event{e}{_1}}{\event{e}{_2}},
% \nBROrdered{\event{e}{_1}}{\event{e}{_2}}, and
% $\commonLocks{\event{e}{_1}}{\event{e}{_2}} = \emptyset$.
Suppose \tr has no predictable race.
Then we want to prove either a contradiction or that \tr has a predictable deadlock.

\sout{If \nHBOrdered{\event{e}{_1}}{\event{e}{_2}}, a predictable race
exists, which is a contradiction. Thus \HBOrdered{\event{e}{_1}}{\event{e}{_2}},
which means there must be a release \event{r}{_1} and acquire \event{a}{_2} such that
\POOrdered{\event{e}{_1}}{\HBOrdered{\event{r}{_1}}{\POOrdered{\event{a}{_2}}{\event{e}{_2}}}}.}
\mike{I don't think that's used later.}

Let \trPrime be a valid reordering of \tr such that:

\begin{itemize}

\item \event{e}{_1}, \event{e}{_2} is the first race in \trPrime;

\item among traces that satisfy the above, the number of events between \event{e}{_1} and \event{e}{_2} is minimized;

\item among traces that satisfy the above, the number of events between any acquire \event{a}{} such that $\event{e}{_1} \in \CS{\event{a}}$
and \event{e}{_2} is minimized, from innermost to outermost acquires; and

\item \event{e}{_2} is the last event of \trPrime.
% (\ie, $\nexists \event{e} \mid \TRPrimeOrdered{\event{e}{_2}}{\event{e}}$).

\end{itemize}

Let us call such a reordering an \emph{extremal trace}.

For the rest of the proof, partial orders \ltHB and \ltBR refer to order in \trPrime (not \tr).

To help prove the theorem, we define and prove the following lemma:

% WCP Lemma 1
\begin{lem}[corresponds to Lemma~A.1 in \cite{wcp}]
  For any event \event{e} such that
  \TRPrimeOrdered{\event{e}{_1}}{\TRPrimeOrdered{\event{e}}{\event{e}{_2}}}, it
  is true that \HBOrdered{\event{e}{_1}}{\HBOrdered{\event{e}}{\event{e}{_2}}},
  \nBROrdered{\event{e}{_1}}{\event{e}}, and
  \nBROrdered{\event{e}}{\event{e}{_2}}.
  \label{lem:hb-between-e1-e2}
\end{lem}

\begin{proof}[Proof of Lemma~\ref{lem:hb-between-e1-e2}]
  Suppose that \nHBOrdered{\event{e}{_1}}{\event{e}} or
  \nHBOrdered{\event{e}}{\event{e}{_2}}. Then a reordering in which \event{e}
  is before \event{e}{_1} or after \event{e}{_2} is valid. Such a
  reordering has fewer events between \event{e}{_1} and \event{e}{_2} than \trPrime,
  contradicting the assumption that \trPrime is extremal.

  Suppose that \BROrdered{\event{e}{_1}}{\event{e}} or
  \BROrdered{\event{e}}{\event{e}{_2}}. Since
  \HBOrdered{\event{e}{_1}}{\event{e}} and \HBOrdered{\event{e}}{\event{e}{_2}},
  by Rule~\ref{br:hb-comp} of \BR,
  \BROrdered{\event{e}{_1}}{\event{e}{_2}}. This contradicts the initial
  assumption that \nBROrdered{\event{e}{_1}}{\event{e}{_2}}.
\end{proof}

% WCP Lemma 2
\begin{lem}[corresponds to Lemma~A.2 in \cite{wcp}]
  Let \event{a}{_1} be an acquire event such that
  \inCS{\event{e}{_1}}{\event{a}{_1}}. For all events \event{e} such that
  \TRPrimeOrdered{\event{a}{_1}}{\TRPrimeOrdered{\event{e}}{\event{e}{_1}}}, it
  must be that \HBOrdered{\event{a}{_1}}{\HBOrdered{\event{e}}{\event{e}{_1}}}.
  \label{lem:hb-between-a1-e1}
\end{lem}

The proof of Lemma~\ref{lem:hb-between-a1-e1} follows the proof used for \CP and \WCP~\cite{causally-precedes,wcp}.

% WCP Lemma 3
\begin{lem}[corresponds to Lemma~A.3 in \cite{wcp}]
  For all pairs of events \event{e}, \event{e}{'} such that
  \TRPrimeOrdered{\event{e}}{\TRPrimeOrdered{\event{e}{'}}{\event{e}{_2}}} and
  \conflicts{\event{e}}{\event{e}{'}}, it must be that
  \BROrdered{\event{e}}{\event{e}{'}} or
  $\commonLocks{\event{e}}{\event{e}{'}}\neq\emptyset$.
  \label{lem:no-earlier-br-race}
\end{lem}

\begin{proof}[Proof of Lemma~\ref{lem:no-earlier-br-race}]
  Otherwise \event{e}, \event{e}{'} is an earlier \BR-race than \event{e}{_1}, \event{e}{_2}.
\end{proof}

We do not attempt to prove a corresponding lemma for \WCP's Lemma~A.4~\cite{wcp}
because the corresponding lemma statement does not hold for \BR.
\mike{That's true even after changing \BR to be have a more conservative rule~(a).
For example, the \WCP Lemma~A.4 counterexample I sent on May 7 still applies with the more conservative rule~(a).}

\begin{lem}
  Let \event{e} be a \CORE write such that
  \TRPrimeOrdered{\event{e}}{\event{e}{_2}}. There must be a branch \event{b} in \trPrime
  such that \BROrdered{\event{e}}{\event{b}}.
  % \mike{I think \TRPrimeOrdered{\event{b}}{\event{e}{_2}} needs to be added to the lemma statement
  % (considering how it's used later; see my later comment)?}
  \label{lem:core-wr-has-br}
\end{lem}

\begin{proof}[Proof of Lemma~\ref{lem:core-wr-has-br}]
  By definition, there must be a \CORE read \event{e}{'} such that
  \conflicts{\event{e}}{\event{e}{'}} and
  \TRPrimeOrdered{\event{e}}{\event{e}{'}}.
%   By Lemma~\ref{lem:core-wr-has-br},
%   \BROrdered{\event{e}}{\event{e}{'}} or $\commonLocks{\event{e}}{\event{e}{'}}\neq\emptyset$.
  % otherwise there is a \BR-race earlier than \event{e}{_1}, \event{e}{_2}.
  Let us proceed by induction on the recursive definition of \event{e}{'} being a \CORE read (Definition~\ref{def:core-event}):

  \paragraph{Base case}

  \event{e}{'} is a \CORE read because there exists a branch event \event{b} such that
  \POOrdered{\event{e}{'}}{\event{b}{}}.
  
  
  By Lemma~\ref{lem:core-wr-has-br},
  \BROrdered{\event{e}}{\event{e}{'}} or $\commonLocks{\event{e}}{\event{e}{'}}\neq\emptyset$.
  If \BROrdered{\event{e}}{\event{e}{'}},
  then \BROrdered{\event{e}}{\event{b}} by \BR \Rule{\ref{br:hb-comp}}. Otherwise
  $\commonLocks{\event{e}}{\event{e}{'}}\neq\emptyset$, and by
  \BR \Rule{\ref{br:wr-rd}} we have \BROrdered{\event{e}}{\event{b}}.

  \paragraph{Inductive case}

  \event{e}{'} is a \CORE read because there exists a \CORE write event \event{e}{''} such that \POOrdered{\event{e}{'}}{\event{e}{''}}.

  By the induction hypothesis, there exists a branch event \event{b} such that \BROrdered{\event{e}{''}}{\event{b}{}}.
  By Lemma~\ref{lem:no-earlier-br-race},
  \HBOrdered{\event{e}}{\event{e}{'}}.
  Applying \BR \Rule{\ref{br:hb-comp}} gives \BROrdered{\event{e}}{\event{b}}.
\end{proof}

% \begin{lem}
%   Let \event{e} be a read or a write event, and \event{r} be a release event
%   such that \inCS{\event{e}}{\event{r}} and for some acquire \event{a}{_1} such
%   that \inCS{\event{e}{_1}}{\event{a}{_1}},
%   \TRPrimeOrdered{\event{a}{_1}}{\TRPrimeOrdered{\event{r}}{\event{e}{_2}}}.
%   Then, \BROrdered{\event{r}}{\event{e}{_2}}.
%   \label{lem:core-ordered-to-e2}
% \end{lem}

% WCP Lemma 4
% \begin{lem}
%   For any critical section $\event{a}\ldots\event{r}$ and
%   acquire event \event{a}{_1} and such that \inCS{\event{e}{_1}}{\event{a}{_1}} and
%   \TRPrimeOrdered{\event{a}}{\TRPrimeOrdered{\event{a}{_1}}{\TRPrimeOrdered{\event{r}}{\event{e}{_1}}}},
%   it must be that \BROrdered{\event{a}{_1}}{\event{r}}.
%   \label{lem:interleaving-rel-ordered}
% \end{lem}
% \mike{I don't understand how this lemma can be true, considering the counterexample to it.
% I see that you changed the overall proof so there's no predictable deadlock---so (assuming the therorem is true)
% there cannot exist any counterexample even if this lemma is false---but somehow that seems too easy. :)
% More precisely, it seems like in order for the lemma to be true in this new context,
% the proof of the lemma would need to use the assumption that there's no predictable deadlock.}

% \begin{proof}[Proof of Lemma~\ref{lem:interleaving-rel-ordered}]
%   Assume that some critical section $\event{a}\ldots\event{r}$ that is
%   \TRPrimeOrdered{\event{a}}{\TRPrimeOrdered{\event{a}{_1}}{\TRPrimeOrdered{\event{r}}{\event{e}{_1}}}}
%   but \nBROrdered{\event{a}{_1}}{\event{r}} exists.

%     Let $\event{a}\ldots\event{r}$ be the critical section that ends the soonest
%   among all critical sections that fit the definition,
%   \mike{Eventually I think this needs to be done by induction, like the CP proof~\cite{causally-precedes}.}
%   and let \event{u} be the
%   first event such that
%   \TRPrimeOrdered{\event{a}{_1}}{\EqPOOrdered{\event{u}}{\event{r}}}. Since
%   \trPrime is an extremal reordering, \trDoublePrime which is same as \trPrime
%   except that $\event{u}\ldots\event{r}$ has been moved to before \event{a}{_1}
%   must be invalid, such a reordering must violate one or more of the rules of a
%   valid reordering. Let us consider the following exhaustive set of cases for
%   possible violations:

%   \paragraph{\PO violations.} Due to well-nestedness of locks, \event{a}{_1} and
%   \event{u} must be on different threads. \nPOOrdered{\event{a}{_1}}{\event{u}}
%   and by definition there is no event \event{u}{'} such that
%   \TRPrimeOrdered{\event{a}{_1}}{\POOrdered{\event{u}{'}}{\event{u}}}, thus such
%   a reordering can not violate \PO rules.

%   \paragraph{\LS violations.} For such a reordering to violate \LS, there must
%   be a critical section $\event{a}{_u}\ldots\event{r}{_u}$ in
%   $\event{u}\ldots\event{r}$. \event{a}{_u} and \event{a}{_1} must be over
%   different locks, otherwise \trPrime would be an invalid reordering. There also
%   must be another critical section $\event{a}{'}\ldots\event{r}{'}$ such that
%   \TRPrimeOrdered{\event{a}{_1}}{\event{r}{'}} and \event{r}{'} releases the
%   same lock \event{a}{_u} acquires, therefore
%   \HBOrdered{\event{r}{'}}{\event{u}}. By definition of
%   $\event{a}\ldots\event{r}$, it must be that
%   \BROrdered{\event{a}{_1}}{\event{r}{'}}. Using rule~\ref{br:hb-comp},
%   \BROrdered{\event{a}{_1}}{\HBOrdered{\event{r}{'}}{\POOrdered{\event{r}{_c}}{\event{r}}}}
%   gives us \BROrdered{\event{a}{_1}}{\event{r}}, which is a contradiction.

%   \paragraph{\LW violations.} For such a reordering to violate \LW, there must
%   exist events \event{e}{'} and \event{e} such that \inCS{\event{e}}{\event{a}},
%   \EqTRPrimeOrdered{\event{u}}{\event{e}} and
%   \conflicts{\event{e}{'}}{\event{e}}. Using lemma~\ref{lem:no-earlier-br-race}
%   it must be \BROrdered{\event{e}{'}}{\event{e}} or
%   $\commonLocks{\event{e}{'}}{\event{u}}\neq\emptyset$. Let us consider these 2
%   subcases:

%   \subparagraph{\BROrdered{\event{e}{'}}{\event{e}}.} There must exist a release
%   \event{r}{_c'} such that
%   \POOrdered{\event{e}{'}}{\BROrdered{\event{r}{_c'}}{\event{e}}}. If
%   \TRPrimeOrdered{\event{r}{_c'}}{\event{a}{_1}}, then a reordering where
%   $\event{u}\ldots\event{r}$ is between \event{r}{_c'} and \event{a}{_1} would
%   be valid, which contradicts that \trPrime is extremal. Otherwise
%   \TRPrimeOrdered{\event{a}{_1}}{\event{r}{_c'}}, and using
%   lemma~\ref{lem:hb-between-a1-e1} we have
%   \HBOrdered{\event{a}{_1}}{\event{r}{_c'}}. Using rule~\ref{br:hb-comp},
%   \HBOrdered{\event{a}{_1}}{\BROrdered{\event{r}{_c'}}{\POOrdered{\event{e}}{\event{r}}}}
%   gives us \BROrdered{\event{a}{_1}}{\event{r}} which is a contradiction.

%   \subparagraph{$\commonLocks{\event{e}{'}}{\event{e}}\neq\emptyset$.} There
%   must exist a release \event{r}{_c'} and an acquire event \event{a}{_c} over
%   the same lock such that \inCS{\event{e}{'}}{\event{r}{_c'}},
%   \inCS{\event{e}}{\event{a}{_c}} and
%   \TRPrimeOrdered{\event{a}{_1}}{\TRPrimeOrdered{\event{r}{_c'}}{\event{a}{_c}}}.
%   Let \event{a}{_c'} and \event{r}{_c} be the matching acquire and release of
%   \event{r}{_c'} and \event{a}{_c} respectively.

%   It may be that \event{e}{'} is a write and \event{e} is a read followed by a
%   dependent branch \event{b} such that \POOrdered{\event{b}}{\event{r}}, or
%   \event{e} is a write and \event{e}{'} is a read followed by a dependent branch
%   \event{b}{'} such that
%   \POOrdered{\event{e}{'}}{\POOrdered{\event{b}{'}}{\event{r}{_c'}}}. Then it
%   must be \BROrdered{\event{r}{_c'}}{\event{r}} using rule~\ref{br:wr-rd} and
%   rule~\ref{br:rd-wr} respectively. By rule~\ref{br:hb-comp} and
%   lemma~\ref{lem:hb-between-a1-e1}, this gives us
%   \BROrdered{\event{a}{_1}}{\event{r}} which is a contradiction.

%   \event{e}{'} and \event{e} may both be writes. There must be a read
%   \event{e}{''} such that \conflicts{\event{e}}{\event{e}{''}} and
%   \TRPrimeOrdered{\event{e}}{\event{e}{''}}.
%   \mike{Should it be the case that \TRPrimeOrdered{\event{e}{''}}{\event{e}{_1}}? Otherwise there's a contradiction immediately.
%   Also, doesn't there need to be a branch after \event{e}{''}?}
%   \HBOrdered{\event{e}}{\event{e}{''}}, otherwise there is a predictable race in
%   \tr. Using Lemma~\ref{lem:core-ordered-to-e2} we have \BROrdered{\event{e}{''}}{\event{e}{_2}}. Using
%   lemma~\ref{lem:hb-between-a1-e1} with rule~\ref{br:hb-comp} we get
%   \BROrdered{\event{a}{_1}}{\event{e}{_2}}. 
%   \kaan{I think the following statement is true, but I don't have a proof for it right now.}
%   There must be a critical section $\event{c}\ldots\event{c}{'}$ such that
%   \BROrdered{\event{e}{_1}}{\HBOrdered{\event{c}{'}}{\event{e}{_2}}}
%   \mike{Isn't that a contradiction right there since \BROrdered{\event{e}{_1}}{\event{e}{_2}}?}
%   and
%   \event{c} acquires the lock $l$ such that $l\in\lockset{\event{e}{_1}}$. Using
%   rule~\ref{br:rule-b} we get \BROrdered{\event{r}{_1}}{\event{c}{'}},
%   \mike{How do we know that \event{r}{_1} isn't really late in \trPrime (it might be after \event{e}{_2}, right)?}
%   and
%   rule~\ref{br:hb-comp} gives us \BROrdered{\event{e}{_1}}{\event{e}{_2}} which is a contradiction.

%   % \mike{In this case, reordering rules wouldn't prevent the reordering, right?
%   % \kaan{Yes, but there may be a conflicting read later that will get a different
%   % last writer if the reordering happens.}
%   % \mike{Ah I see. These cases seem hard. Are we sure the theorem is true?
%   % Will \CORE events be used to restate the theorem or just for the proof?}}

%   One of them may be a read that has no dependent branch. In that case, the
%   reordering does not violate \LW and is valid, meaning that \trPrime is not
%   extremal which is a contradiction.

%   One of them may be a read that has a dependent branch, but after
%   \event{r}{_c'} or \event{r}. Let \event{b} be that branch event. Using
%   lemma~\ref{lem:core-ordered-to-e2} have \BROrdered{\event{b}}{\event{e}{_2}},
%   \mike{How can Lemma~\ref{lem:core-ordered-to-e2} be used to show that? Event \event{b} isn't necessarily inside any critical section.}
%   which means
%   \BROrdered{\event{r}{_c'}}{\event{e}{_2}}. Rest of proof for this sub-subcase
%   is same as branch being within the critical section.
%   \mike{I don't understand how the rest of the proof goes.}
% \end{proof}
%
% The lemma seem to be incorrect. Even if we add write-write edges, the same
% issue exists for reads that have a dependent branch that is outside their
% critical section.

% WCP Lemma 5
\begin{lem}[Corresponds to Lemma~A.5 in \cite{wcp}]
  Let \event{a} be an acquire event, and \event{r} be the matching release
  event. If \TRPrimeOrdered{\event{e}{_1}}{\event{a}} and
  $\event{r}\not\in\trPrime$, then \inCS{\event{e}{_2}}{\event{a}}.
  \label{lem:no-unfinished-cs-outside-e2}
\end{lem}

\begin{proof}[Proof of Lemma~\ref{lem:no-unfinished-cs-outside-e2}]
  Assume that an acquire event \event{a} exists such that
  \TRPrimeOrdered{\event{e}{_1}}{\event{a}{}} and the matching release
  $\event{r}{}\not\in\trPrime$, but $\event{e}{_2}\not\in\CS{\event{a}}$.
%  \mike{What exactly are you assuming here? Assuming \nPOOrdered{\event{a}}{\event{e}{_2}} for a contradiction proof?}
%  Let \event{a} be the last acquire event among all acquires that fit the definition of \event{a}{'}.
%  \mike{Why assuming the latest---does proof use that? Assuming latest means proof isn't complete, right?}
  Let \event{u} be the last event such that
  \POOrdered{\event{a}}{\TRPrimeOrdered{\event{u}}{\event{e}{_2}}}. Then,
  consider a reordering \trDoublePrime which is the same as \trPrime except that
  $\event{a}\ldots\event{u}$ (a segment of events from the same thread)
  has been removed. Such a reordering must violate
  one of the rules of a valid reordering (Definition~\ref{def:valid-reordering}), because otherwise \trPrime would not be extremal.

  \paragraph{\trDoublePrime violates \PO}

  Since there is no event \event{e} in \trPrime such that \POOrdered{\event{u}}{\event{e}}
  (note that \nPOOrdered{\event{u}}{\event{e}{_2}} because $\event{e}{_2}\not\in\CS{\event{a}}$),
  \trDoublePrime does not violate \PO.

  \paragraph{\trDoublePrime violates \LS}

  Due to the well-nestedness of locks, there can not be any critical section
  that ends before \event{u} but starts before \event{a}. Therefore, for any
  release event we remove, we also remove the matching acquire event. As a
  result, \trDoublePrime does not violate \LS.

  \paragraph{\trDoublePrime violates \LW}

  In order for a \CORE read to have a different last writer in \trDoublePrime than in \trPrime,
  there must be a \CORE write \event{e}
  such that \TRPrimeOrdered{\event{a}{}}{\event{e}{}}. Using Lemma~\ref{lem:core-wr-has-br},
  there must be a branch \event{b} in \trPrime such that \BROrdered{\event{e}}{\event{b}}.
  By definition, \TRPrimeOrdered{\event{b}}{\event{e}{_2}} otherwise \event{b} would not exist in \trPrime.
  % \mike{It seems like we need \TRPrimeOrdered{\event{b}}{\event{e}{_2}} too?
  % As is, there seems to be an assumption that \trPrime ends at \event{e}{_2} and that $\event{b} \in \trPrime$
  % (which is another way to go, I suppose, but needs to be more explicitly stated).}
  Using either Lemma~\ref{lem:hb-between-e1-e2}
  \sout{or Lemma~\ref{lem:hb-between-a1-e1}},
  \mike{How does it follow from Lemma~\ref{lem:hb-between-a1-e1}?}
  we have \HBOrdered{\event{e}{_1}}{\event{e}}
  and \HBOrdered{\event{b}}{\event{e}{_2}}. Using \BR \Rule{\ref{br:hb-comp}},
  \BROrdered{\event{e}{_1}}{\event{e}{_2}}, which is a contradiction.

  \medskip
  \noindent
  Therefore, \trDoublePrime cannot be invalid, which violates the extremality of \trPrime, a contradiction.
%   As a result, $\event{e}{_2} \in \CS{\event{a}}$.
\end{proof}

Let \event{f} be the first event such that
\TRPrimeOrdered{\event{e}{_1}}{\event{f}} and
\nPOOrdered{\event{e}{_1}}{\event{f}}. Using Lemma~\ref{lem:hb-between-e1-e2},
\event{f} must be an acquire event and there must be a release event
\event{g}{'} over the same lock such that
\POOrdered{\event{e}{_1}}{\event{g}{'}}. Let \event{g} be the matching acquire
event of \event{g}{'}. If the matching release of \event{f} exists, let that
event be \event{f}{'}.

Among all extremal traces, we now (potentially) redefine \trPrime to be a trace that has the fewest events
between \event{e}{_1} and \event{f}. We call such a reordering of \tr a \emph{minimal trace}.

\mike{After this point, the \emph{\WCP proof} refers to both the extremal trace and the minimal trace.
Why do the authors do that?
Instead, we're just dealing with the minimal trace since it's also an extremal trace.}

% WCP Lemma 8
\begin{lem}[corresponds to Lemma~A.8 in \cite{wcp}]
  If \inCS{\event{e}{_1}}{\event{g}} then $\event{f}{'}\in\trPrime$.
  \label{lem:fprime-exists-if-e1-in-g}
\end{lem}

\begin{proof}
  Suppose that $\event{f}{'}\not\in\trPrime$.
  Then using Lemma~\ref{lem:no-unfinished-cs-outside-e2},
  \inCS{\event{e}{_2}}{\event{f}}. Since \inCS{\event{e}{_1}}{\event{g}}, and
  \event{f} and \event{g} are over the same lock, \event{e}{_1} and
  \event{e}{_2} are not a \BR-race, which is a contradiction.
\end{proof}

% WCP Lemma 6
\begin{lem}[corresponds to Lemma~A.6 in \cite{wcp}]
  If there are events \event{e} and \event{e}{'} such that
  \BROrdered{\event{e}}{\event{e}{'}}, \TRPrimeOrdered{\event{g}}{\event{e}}, and
  $\HBOrdered{\event{e}{'}}{\event{f}{'}} \lor \event{f}{'}\not\in\trPrime$,
%   and one of the following holds: (i) \HBOrdered{\event{e}{'}}{\event{f}{'}} or (ii) $\event{f}{'}\not\in\trPrime$,
  then \BROrdered{\event{e}{_1}}{\event{e}{_2}}.
%   \mike{But that's a contradiction---is this the intended lemma statement?
%     \kaan{This is the statement used by \WCP. I think we should instead say that
%       if \BROrdered{\event{e}}{\event{e}{'}},
%       \TRPrimeOrdered{\event{g}}{\event{e}} then $\event{f}{'}\in\trPrime$ and
%       \HBOrdered{\event{e}{'}}{\event{f}{'}}. Is that equivalent?}
%     \mike{Ah okay, I think it's okay without that change (but it's okay to modify it if that helps somehow).
%     I modified it a bit to look more like \WCP's proof.}}
  \label{lem:no-br-after-g}
\end{lem}

\begin{proof}[Proof of Lemma~\ref{lem:no-br-after-g}]
  We consider the possible orders of \event{e}{_1} and \event{g}{} as separate cases:

  \begin{enumerate}
  \item \POOrdered{\event{e}{_1}}{\event{g}}. Then
    \TRPrimeOrdered{\event{e}{_1}}{\TRPrimeOrdered{\event{e}}{\event{e}{'}}},
    and using Lemma~\ref{lem:hb-between-e1-e2} we have
    \HBOrdered{\event{e}{_1}}{\event{e}} and
    \HBOrdered{\event{e}{'}}{\event{e}{_2}}. Thus
    \HBOrdered{\event{e}{_1}}{\BROrdered{\event{e}}{\HBOrdered{\event{e}{'}}{\event{e}{_2}}}},
    which using \BR \Rule{\ref{br:hb-comp}} gives us \BROrdered{\event{e}{_1}}{\event{e}{_2}}.
  \item \POOrdered{\event{g}}{\event{e}{_1}}.
    By Lemma~\ref{lem:hb-between-a1-e1},
    \HBOrdered{\event{g}}{\event{e}}.
    According to Lemma~\ref{lem:fprime-exists-if-e1-in-g}, $\event{f}{'}\in\trPrime$,
    so \HBOrdered{\event{e}{'}}{\event{f}{'}}.
    Thus we have
    \HBOrdered{\event{g}}{\BROrdered{\event{e}}{\HBOrdered{\event{e}{'}}{\event{f}{'}}}}, and
    using \BR \Rule{\ref{br:hb-comp}} gives us \BROrdered{\event{g}}{\event{f}{'}}.
    Using \BR \Rule{\ref{br:rule-b}} we get \BROrdered{\event{g}{'}}{\event{f}{'}}.
    By Lemma~\ref{lem:hb-between-e1-e2}, \HBOrdered{\event{f}{'}}{\event{e}{_2}}.
    Thus \POOrdered{\event{e}{_1}}{\BROrdered{\event{g}{'}}{\HBOrdered{\event{f}{'}}{\event{e}{_2}}}},
    which using \BR \Rule{\ref{br:hb-comp}}
    gives us \BROrdered{\event{e}{_1}}{\event{e}{_2}}.
  \end{enumerate}
  
Thus in both cases, \BROrdered{\event{e}{_1}}{\event{e}{_2}}.
\end{proof}

\newcommand{\Tau}{\ensuremath{\tau}\xspace}
\newcommand{\TauPrime}{\ensuremath{\tau'}\xspace}
\newcommand{\ltTau}{\ensuremath{<_\textsc{\Tau}}\xspace}
\newcommand{\ltTauPrime}{\ensuremath{<_\textsc{\TauPrime}}\xspace}
\newcommand{\TauOrdered}[2]{\Ordered{#1}{\ltTau}{#2}}
\newcommand{\TauPrimeOrdered}[2]{\Ordered{#1}{\ltTauPrime}{#2}}

\begin{definition}[Lockset violations]
  Given a trace \Tau,
  let $\event{a}\ldots\event{b}$ be a segment of events from the same thread,
  and let \event{c} be an event by a different thread such that \TauOrdered{\event{c}}{\event{a}}.
  Consider a reordering \TauPrime that is the same as \Tau except that
  $\event{a}\ldots\event{b}$ is moved just before \event{c}. If \TauPrime
  violates the \LS rule for a valid reordering, there are two possibilities:

  \begin{enumerate}
  \item $\event{a}\ldots\event{b}$ contains a critical section
    $\event{d}\ldots\event{d}{'}$, and there exists an acquire \event{h} such
    that \inCS{\event{c}}{\event{h}}, and \event{h} and \event{d} acquire the
    same lock. Let us call this an \emph{\LSOne violation}.
  \item $\event{a}\ldots\event{b}$ contains an acquire \event{d}, but not the
    matching release \event{d}{'}, and there exists a critical section
    $\event{h}\ldots\event{h}{'}$ in another thread that is over the same lock
    and \TauOrdered{\event{c}}{\POOrdered{\event{h}}{\TauOrdered{\event{h}{'}}{\event{d}}}}.
    Let us call this an \emph{\LSTwo violation}.
  \end{enumerate}
\end{definition}

% WCP Lemma 7
\begin{lem}[corresponds to Lemma~A.7 in \cite{wcp}]
  Given a trace \Tau,
  let $\event{a}\ldots\event{b}$ be a segment of events in a thread such that
  for every acquire \event{d} in the segment the matching release \event{d}{'}
  is also in the segment, and let \event{c} be an event such that
  \TauOrdered{\event{c}}{\event{a}}. Let \TauPrime be a reordering that is same as
  \Tau, except that $\event{a}\ldots\event{b}$ is moved to just before \event{c}.
  \TauPrime can not violate \LSTwo.
  \label{lem:no-ls2-for-suffix-move}
\end{lem}

\begin{proof}[Proof of Lemma~\ref{lem:no-ls2-for-suffix-move}]
  Trivially, the segment does not contain any acquire \event{d} for which the
  matching release \event{d}{'} is not in the segment, so \LSTwo cannot be
  violated.
\end{proof}

\begin{definition}[corresponds to Definition~4 in \cite{wcp}]
  A critical section $(\event{c}, \event{c}{'})$ such that
  \TRPrimeOrdered{\event{g}}{\event{c}} is said to be conflicting due to
  critical section $(\event{d}, \event{d}{'})$ if \event{d} and \event{c}
  acquire the same lock and
  \TRPrimeOrdered{\event{d}}{\TRPrimeOrdered{\event{g}}{\HBOrdered{\event{d}{'}}{\event{c}}}}.
  \label{def:cs-conflicts-one}
\end{definition}

\begin{definition}[corresponds to Definition~5 in \cite{wcp}]
  A \emph{deadlock chain of type 1 and length k} is a sequence of threads $v_1
  \dots v_{k+1}$ and sequence of critical sections $(\event{c}{_1},
  \event{c}{_1'}), (\event{d}{_1}, \event{d}{_1'}), \dots , (\event{c}{_k},
  \event{c}{_k'}), (\event{d}{_k}, \event{d}{_k'})$ such that

  \begin{enumerate}
  \item $v_1 \dots v_{k+1}$ are distinct, and $t \notin \{v_1 \dots v_{k}\}$ where $t$ is \event{e}{_1}'s thread.
  \item $\event{f} \in v_1$
  \item $\forall i : (\event{c}{_i}, \event{c}{_i'})$ is the earliest critical
    section such that $\event{c}{_i} \in (\event{d}{_{i-1}},
    \event{d}{_{i-1}'})$, or $\event{c}{_i} \in (\event{f}, \event{f}{'})$ if $i=1$
  \item $\forall i : (\event{c}{_i}, \event{c}{_i'})$ conflicts due to $(\event{d}{_i}, \event{d}{_i'})$
  \item $\forall i : \event{d}{_i} \in v_i$
  \end{enumerate}
  \label{def:deadlock-chain-one}
\end{definition}

\begin{definition}[corresponds to Definition~6 in \cite{wcp}]
  An acquire event \event{d} is said to be conflicting due to a critical section
  $(\event{c}, \event{c}{'})$ if $\event{e}{_1} \in (\event{g}, \event{g}{'})$,
  \event{c} and \event{d} acquire the same lock, and
  \TRPrimeOrdered{\event{d}}{\TRPrimeOrdered{\event{g}}{\HBOrdered{\event{d}{'}}{\event{c}}}}.
  \label{def:cs-conflicts-two}
\end{definition}

\begin{definition}[corresponds to Definition~7 in \cite{wcp}]
  A \emph{deadlock chain of type 2} and length $k$ is a sequence of threads $v_1
  \dots v_{k+1}$ and sequence of critical sections $(\event{c}{_1},
  \event{c}{_1'}), (\event{d}{_1}, \event{d}{_1'}), \dots , (\event{c}{_k},
  \event{c}{_k'}), (\event{d}{_k}, \event{d}{_k'})$ such that

  \begin{enumerate}
  \item $v_1 \dots v_{k+1}$ are distinct, and $t \notin \{v_1 \dots v_{k}\}$ where $t$ is \event{e}{_1}'s thread.
  \item $\event{f} \in v_1$ and $\event{f} \in (\event{d}{_1}, \event{d}{_1'})$
  \item $\forall i : (\event{d}{_i}, \event{d}{_i'})$ is the earliest critical
    section such that $\event{c}{_{i-1}} \in (\event{d}{_i}, \event{d}{_i'})$, or
    $\event{f} \in (\event{d}{_i}, \event{d}{_i'})$ if $i=1$
  \item $\event{d}{_i}$ is conflicting due to $(\event{c}{_i}, \event{c}{_i'})$
  \item $\event{c}{_i} \in v_{i+1}$
  \end{enumerate}
\end{definition}

\begin{lem}[corresponds to Lemma~A.9 in \cite{wcp}]
The minimal trace \trPrime contains a deadlock chain of type 1 or type 2.
\label{lem:trPrime-has-deadlock-chain}
\end{lem}

\begin{proof}[Proof of Lemma~\ref{lem:trPrime-has-deadlock-chain}]
Consider two exhaustive cases:
\begin{enumerate}

\item $\event{f}{'} \in \trPrime$. \ldots

\item $\event{f}{'} \notin \trPrime$. \ldots

\end{enumerate}
\end{proof}

\mike{The rest of the corresponding lemmas in the \WCP proof show that a deadlock chain implies a predictable deadlock.
The proofs of those lemmas rely on \WCP Lemma~A.4 (which doesn't hold for \BR),
and perhaps they rely on some other differences of \WCP vs.\ \BR?
Or is there something I'm missing that means that a deadlock chain implies a predictable deadlock regardless of whether we're in
the \WCP vs.\ \BR soundness proof?}

By Lemmas~\ref{??}\ldots
\end{proof}

% \end{empty}


==> Old-Wr-Wr-Conflict.tex <==
%auto-ignore

\small
\centering

\subfloat[Execution with \WBR-race but no \DC-race]{
\centering
\sf
\makebox[.5\linewidth]{
\begin{tabular}{@{}lll@{}}
\textnormal{Thread 1} & \textnormal{Thread 2} & \textnormal{Thread 3}\\\hline
\Acquire{m} \\
\Write{x} \\
\Write{y} \\
\Release{m}\tikzmark{3} \\
					  & acq(m) \\
				 	  & \tikzmark{4}wr(x) \\
					  & rel(m)\tikzmark{1} \\
                      &						  & acq(m) \\
                      &						  & \tikzmark{5}rd(x) \\
                      &						  & \tikzmark{2}\BrUniv \\
                      & 					  & rel(m) \\
                      &						  & rd(y) \\
%                       &						  & \\
\end{tabular}}
\label{fig:wr-wr-conflict:original}}
\subfloat[Valid reordering of (a) demonstrating that (a) has a predictable race]{
\centering
\sf
\makebox[.5\linewidth]{
\begin{tabular}{@{}lll@{}}
\textnormal{Thread 1} & \textnormal{Thread 2} & \textnormal{Thread 3}\\\hline
					  & acq(m) \\
				 	  & wr(x) \\
					  & rel(m) \\
                      &						  & acq(m) \\
                      &						  & rd(x) \\
                      &						  & \BrUniv \\
                      & 					  & rel(m) \\
\Acquire{m} \\
\Write{x} \\
\Write{y} \\
                      &						  & rd(y) \\
\\
% \\
\end{tabular}}
\label{fig:wr-wr-conflict:reordered}}
\textlink{1}{5}{\DC}%
\textunderlink{1}{2}{\WBR}%
\textlink{3}{4}{\DC}%

\mike{The execution has no \BR-race. Presumably we want a (write--write) example
that shows a case where \BR finds a race that \WCP (and \DC?) don't find.}

\caption{Example showing \DC's overly strict handling of write--write dependencies.
% The example execution in (a) has no \DC-race 
% (\eg, \WCPOrdered{\Write{y}{}}{\Read{y}{}}), 
% but it has a predictable race
% % since write--read order on \code{x} is preseved in \trPrime, 
% as the reordered execution in (b) demonstrates.
\label{fig:wr-wr-conflict}}
% \jake{I'm not sure if this example is correct or not. Would this be successfully Vindicated?
%   \kaan{This is actually not a \WBR race, see the edge I added. This is actually
%     a counterexample for \WBR's completeness: we should only have wr-rd edges
%     for the last writer of the read.}
%     \jake{The added edge should be removed with the latest change to \WBR
%     completeness, right?}
%     \mike{Yeah; removed it.}}
% \jake{I'm adding the \CORE example to the wr-wr-conflict example. 
% Not sure if this is an overloaded example,
% but the figures are similar and there is room so I put it here.
% \mike{Overloading (a) for showing both \CORE events and why \WBR is unsound, seems good to me.
% However, (a) seems separate from (b) and (c), right? I think it should be a separate figure (can still be side-by-side).}
% \mike{Applied}}


==> WBR-incomplete.tex <==
%auto-ignore
\begin{figure}

\small
\centering

\subfloat[\WBR rule (b)'s composition with FD causes incompleteness]{
\centering
\sf
\makebox[.4\linewidth]{
\begin{tabular}{@{}lll@{}}
\textnormal{Thread 1} & \textnormal{Thread 2} & \textnormal{Thread 3} \\\hline 
wr(z)                 &                       &                       \\
acq(o)                &                       &                       \\
wr(y)                 &                       &                       \\
rel(o)\tikzmark{1}    &                       &                       \\
                      & acq(m)                &                       \\
                      & acq(n)                &                       \\
                      & wr(x)                 &                       \\
                      & rel(n)\tikzmark{3}    &                       \\
                      & acq(o)                &                       \\
                      & \tikzmark{2}rd(y)     &                       \\
                      & rel(o)                &                       \\
                      & \tikzmark{5}rel(m)    &                       \\
                      &                       & acq(m)                \\
                      &                       & acq(n)                \\
                      &                       & rd(x)                 \\
                      &                       & \tikzmark{4}\BrUniv   \\
                      &                       & rel(n)                \\
                      &                       & \tikzmark{6}rel(m)    \\
                      &                       & wr(z)                 
\end{tabular}}
\label{fig:WBR-incomplete:rule-b}}
\textlink{1}{2}{FD}
\textlink{3}{4}{\WBR}
\textlink{5}{6}{\WBR (\ref{wbr:rule-b})}
%\textlink{1}{6}{\WBR (\ref{wbr:dc-left})}
\subfloat[\WBR rule (a)'s composition with FD causes incompleteness]{
\centering
\sf
\makebox[.4\linewidth]{
\begin{tabular}{@{}lll@{}}
\textnormal{Thread 1} & \textnormal{Thread 2} & \textnormal{Thread 3} \\\hline 
wr(z)                 &                       &                       \\
acq(o)                &                       &                       \\
wr(y)                 &                       &                       \\
rel(o)\tikzmark{10}   &                       &                       \\
                      & acq(m)                &                       \\
                      & wr(x)                 &                       \\
                      & acq(o)                &                       \\
                      & \tikzmark{11}rd(y)    &                       \\
                      & rel(o)                &                       \\
                      & rel(m)\tikzmark{12}   &                       \\
                      &                       & acq(m)                \\
                      &                       & rd(x)                 \\
                      &                       & \tikzmark{13}\BrUniv  \\
                      &                       & rel(m)                \\
                      &                       & wr(z)                 \\
                      \\
                      \\
                      \\
                      \\
\end{tabular}}
\label{fig:WBR-incomplete:rule-a}}

\textlink{10}{11}{FD}
\textlink{12}{13}{\WBR (\ref{wbr:wr-rd})}
%\textlink{10}{13}{\WBR (\ref{wbr:dc-left})}

\caption{There is a predictable race on \emph{z} in both examples.
  Rule{\ref{wbr:dc-left}} edges have been omitted, but they order the accesses on
  z in both examples.}
\label{fig:WBR-incomplete}
\jake{Does FD stand for Flow Dependency? Also, these examples do not hold with the changes to \WBR definition, right?
\mike{Right. Removed this figure from the paper.}}
\end{figure}


==> WBR-only-BR-only-rdwr.tex <==
%auto-ignore
\begin{figure}

\small
\centering

\subfloat[\WCP and \DC miss a predictable race]{
\centering
\sf
\makebox[.3\linewidth]{
\begin{tabular}{@{}ll@{}}
\textnormal{Thread 1} & \textnormal{Thread 2} \\\hline 
acq(m)                & \\
rd(x)                 & \\
wr(y)                 & \\
rel(m)\tikzmark{1}    & \\
                      & acq(m) \\
                      & \tikzmark{2}wr(x) \\
                      & rel(m) \\
                      & wr(y) \\
                      & \\
\end{tabular}}
\label{fig:WCP-DC-misses-race-rdwr}}
\hfill
\subfloat[\BR misses a predictable race]{
\centering
\sf
\makebox[.3\linewidth]{
\begin{tabular}{@{}ll@{}}
\textnormal{Thread 1} & \textnormal{Thread 2} \\\hline 
acq(m)                & \\
rd(x)                 & \\
wr(y)                 & \\
\BrUniv               & \\
rel(m)\tikzmark{3}    & \\
                      & acq(m) \\
                      & wr(x) \\
                      & \tikzmark{4}rel(m) \\
                      & wr(y) \\
\end{tabular}}
\label{fig:BR-misses-race-rdwr}}
\hfill
\subfloat[\WBR reports a false race]{
\centering
\sf
\makebox[.3\linewidth]{
\begin{tabular}{@{}ll@{}}
\textnormal{Thread 1} & \textnormal{Thread 2} \\\hline 
acq(m)                & \\
rd(x)                 & \\
\BrUniv               & \\
wr(y)                 & \\
rel(m)\tikzmark{5}    & \\
                      & acq(m) \\
                      & wr(x) \\
                      & \tikzmark{6}rel(m) \\
                      & wr(y) \\
\end{tabular}}
\label{fig:WBR-false-race-rdwr}}

\textlink{1}{2}{\DC}%
\textlink{3}{4}{\BR}%
\textlink{5}{6}{\BR}%

\mike{Labeled each edge with the weakest relation that holds,
since stronger relations inherently hold. That probably needs some explanation.}

\mike{I think the consensus is that we can remove this example, in favor of (a revised version of) Figure~\ref{fig:br-rd-wr-conflict}.}

\caption{There is a predictable race on \texttt{y} in (a) and (b), but not in
  (c). In both (a) and (b), if the order of the critical sections were flipped
  the write to y would still be observed even though the value read by x is
  different, since there is no branch event before it. However in (c) the branch
  event may change the execution and skip the write to y, in which case no race
  would occur. \WCP and \DC miss the race in (a) and (b), and \BR misses the race in
  (b). \WBR is able to detect all of these races, but also detects the false
  race in (c).}
\end{figure}


==> WBR-only-left-composition.tex <==
%auto-ignore
\begin{figure}

\small
\centering

\subfloat[\BR misses the predictable race]{
\centering
\sf
\makebox[.4\linewidth]{
\begin{tabular}{@{}lll@{}}
\textnormal{Thread 1} & \textnormal{Thread 2} & \textnormal{Thread 3} \\\hline 
acq(m)                &                       &                       \\
wr(x)                 &                       &                       \\
rel(m)\tikzmark{1}    &                       &                       \\
                      & \tikzmark{0}acq(m)    &                       \\
                      & sync(p)\tikzmark{2}   &                       \\
                      &                       & \tikzmark{3}sync(p)   \\
                      &                       & wr(x)                 \\
                      & sync(p)\tikzmark{4}   &                       \\
                      & rel(m)                &                       \\
                      &						  &						  \\
                      &						  &						  \\
\end{tabular}}
\label{fig:HB-composition-necessary:race}}
% %
% \subfloat[A false race that \BR would detect if it did not compose with \HB]{
\subfloat[\BR correctly detects no predictable race]{
\centering
\sf
\makebox[.4\linewidth]{
\begin{tabular}{@{}lll@{}}
\textnormal{Thread 1} & \textnormal{Thread 2} & \textnormal{Thread 3} \\\hline 
acq(m)                &                       &                       \\
wr(x)                 &                       &                       \\
sync(o)               &                       &                       \\
rel(m)\tikzmark{6}    &                       &                       \\
                      & \tikzmark{7}acq(m)    &                       \\
                      & sync(p)\tikzmark{8}   &                       \\
                      &                       & \tikzmark{9}sync(p)   \\
                      &                       & wr(x)                 \\
                      & sync(p)\tikzmark{10}  &                       \\
                      & \tikzmark{11}sync(o)  &                       \\
                      & rel(m)                &                       
\end{tabular}}
\label{fig:HB-composition-necessary:no-race}}

% \kaan{I was trying to put these side by side, but I can't seem to get it to work.
% \mike{Fixed it. The trick was leaving no empty line between the subfloats.}}

\mike{``Any\ldots\ must\ldots'' seems too strong in the caption. Or is there a reason we can say that?}

\mike{These examples would apply to \WCP, not just \BR.
It seems to me that for \BR, \HB composition doesn't just help with the \LS rule (which is its sole benefit for \WCP),
but it also allows \BR to not order write--write conflicts.
It may likewise help weaken the ordering of read--write conflicts (compared with \WCP).}

\jake{The second sync(p) in Thread 2 for both examples are unnecessary to make the point that \BR is sound but misses races due to composition with \HB.}

\mike{In any case, this example is outside the scope of a \WBR-only paper, so ignoring it for now.}

\textlink{1}{0}{\HB}
\textlink{2}{3}{\BR}
\textlink{3}{4}{\BR}

\textlink{6}{7}{\HB}
\textlink{8}{9}{\BR}
\textlink{9}{10}{\BR}
\textlink{6}{11}{\BR}

\caption{sync(o) represents the series of events
  \{acq(o);rd(oVar);\BrUniv;wr(oVar);rel(o)\}, similar for sync(p). There is a
  predictable race on \texttt{x} in (a), but not in (b). Any online predictive
  race detection method using a partial order must compose with \HB in order to
  avoid reporting the false race in (b): At the write to \texttt{x} by Thread 3,
  the relation must decide if there will be an ordering from the critical
  section in Thread 1 to the ongoing critical section in Thread 2. Without
  future information, the relation must either assume that there will be an
  ordering (in which case it will miss the race in (a)), or assume that there
  will be no ordering (in which case it will report the false race in (b)).}
\end{figure}


==> WBR-pseudo-soundness-proof.tex <==
%auto-ignore
\section{\WBR Pseudo-Soundness Proof}
\label{sec:wbr-pseudo-soundness-proof}

\mike{We don't necessarily need pseudo-soundness as a property in this paper, right?
It's perhaps interesting and useful to use a pseudo-sound relation, but not essential
as long as AddConstraints+ConstructReorderedTrace are strong enough to ensure correctness.}

% \WDC is able to detect data races in real programs without false positives, even
% though it is unsound.
% \mike{Huh?}
We define the property \emph{\psoundness} for race
detection methods. We believe that relations that fit this definition will be
able detect data races in real programs without false positives.
\mike{Oh okay, I see what you're saying, but we should be careful how we pitch this.}
 
\begin{definition}[\Pvalid reordering]
  Given a trace \tr, a reordering \trPrime is \pvalid if it is valid except
  for \LS rule of valid reordering rules.
\end{definition}

\begin{definition}[\Ppredictable race]
  Given a trace \tr, for some events \event{e} and \event{e}{'} such that
  \conflicts{\event{e}}{\event{e}{'}} and
  $\commonLocks{\event{e}{}}{\event{e}{'}} = \emptyset$, if a pseudo-valid
  reordering \trPrime exists where \event{e} and \event{e}{'} are consecutive,
  then a pseudo-predictable race exists in \tr.
\end{definition}

Given an execution \tr, let a \emph{pseudo-predictable race} be a race (consecutive conflicting accesses) that occurs in a
pseudo-valid reordering \trPrime.

A race detection method is \emph{\psound} if it only reports
pseudo-predictable races.

To prove that \WBR is pseudo-sound, we first prove that \DC is pseudo-sound.

\mike{Since \WBR doesn't actually left-compose with full \DC (it composes with something weaker),
then proving \DC pseudo-soundness presumably isn't directly helpful anymore. Instead we should prove the pseudo-soundness of the weaker relation, right?
We could also keep the proof of \DC pseudo-soundness (which is actually pretty trivial if we can prove pseudo-soundness of a weaker relation),
since that's a (small) contribution on its own.}

\begin{thm}[\DC pseudo-soundness]
  If an execution \tr has a \DC-race,
  then it has a pseudo-predictable race.
\label{thm:dc-pseudo-sound}
\end{thm}

\begin{proof}
  Let us prove the theorem by contradiction. Suppose that there is an execution
  \tr with a \DC-race but \emph{no} pseudo-predictable race. Let \event{e}{_1}
  and \event{e}{_2} be the \emph{first} \DC-race in \tr. So
  \TROrdered{\event{e}{_1}}{\event{e}{_2}},
  \conflicts{\event{e}{_1}}{\event{e}{_2}},
  \nDCOrdered{\event{e}{_1}}{\event{e}{_2}},
  and there does not
  exist a \DC-race \nWDCOrdered{\event{e}{}}{\event{e}{'}} such that
  \TROrdered{\event{e}{'}}{\event{e}{_2}} nor a \DC-race
  \nWDCOrdered{\event{e}{}}{\event{e}{_2}} such that
  \TROrdered{\event{e}{_1}}{\event{e}{}}.

  Let \trPrime be a pseudo-valid minimal reordering of \tr such that the number
  of events between \event{e}{_1} and \event{e}{_2} are minimized across all
  pseudo-valid reorderings. As there is no pseudo-predictable race in the
  execution, there must be some event \event{e} such that
  \TRPrimeOrdered{\event{e}{_1}}{\TRPrimeOrdered{\event{e}}{\event{e}{_2}}},
  otherwise a pseudo-valid reordering where a race occurs exists which is a contradiction.

  \trPrime is pseudo-valid and minimal in respect to \event{e}{_1} and
  \event{e}{_2}, and
  \TRPrimeOrdered{\event{e}{_1}}{\TRPrimeOrdered{\event{e}}{\event{e}{_2}}}.
  Therefore using Lemma~\ref{lem:dc-between-e1-e2},
  \mike{Note that the Lemma~\ref{lem:wbr:dc-between-e1-e2} proof now uses this theorem (it seemed necessary to me),
  so this proof can't use Lemma~\ref{lem:wbr:dc-between-e1-e2}.}
  it must be true that
  \DCOrdered{\event{e}{_1}}{\DCOrdered{\event{e}}{\event{e}{_2}}}. Then using
  rule (d) of \DC we have \DCOrdered{\event{e}{_1}}{\event{e}{_2}}, which is a
  contradiction of our initial assumption.
\end{proof}

\begin{thm}[\WBR pseudo-soundness]
  If an execution \tr has a \WBR-race,
  then it has a pseudo-predictable race.
  \label{thm:wbr-pseudo-sound}
\end{thm}

\begin{proof}

Let us prove the theorem by contradiction. Suppose that there is an execution \tr
with a \WBR-race but \emph{no} pseudo-predictable race.
Let \event{e}{_1} and \event{e}{_2} be the \emph{first} \WBR-race in \tr.
So
\TROrdered{\event{e}{_1}}{\event{e}{_2}},
\conflicts{\event{e}{_1}}{\event{e}{_2}},
\nWBROrdered{\event{e}{_1}}{\event{e}{_2}},
$\commonLocks{\event{e}{_1}}{\event{e}{_2}} = \emptyset$,
and there does not exist a \WBR-race \nWBROrdered{\event{e}{}}{\event{e}{'}} such that \TROrdered{\event{e}{'}}{\event{e}{_2}}
nor a \WBR-race \nWBROrdered{\event{e}{}}{\event{e}{_2}} such that
\TROrdered{\event{e}{_1}}{\event{e}{}}.
\kaan{I don't think we ever rely on the assumption that there are no earlier
  \WBR-races, just that there are no pseudo-predictable races. Same for \DC's
  pseudo-soundness proof.}

If \nDCOrdered{\event{e}{_1}}{\event{e}{_2}}, then
by Theorem~\ref{thm:dc-pseudo-sound}, there would be a pseudo-predictable race,
which is a contradiction.
Thus \DCOrdered{\event{e}{_1}}{\event{e}{_2}}.

\paragraph{Minimal reordering.}

Let \trPrime be a pseudo-valid reordering of \tr such that the number of events
between \event{e}{_1} and \event{e}{_2} is minimized among all pseudo-valid
reorderings of \tr, and \event{e}{_2} is the last event in \trPrime
(i.e., $\nexists \event{e} \mid \TRPrimeOrdered{\event{e}{_2}}{\event{e}}$).
Let us call such a reordering a \emph{minimal reordering}.

Since \tr does not have a pseudo-predictable race,
\event{e}{_1} and \event{e}{_2} cannot be consecutive in \trPrime,
i.e., $\exists \event{e}{} \mid \TRPrimeOrdered{\event{e}{_1}}{\TRPrimeOrdered{\event{e}{}}{\event{e}{_2}}}$.

% To prove the theorem, we
% must show that the initial assumptions lead to contradiction by showing that
% \WBROrdered{\event{e}{_1}}{\event{e}{_2}} or that there are no events between
% \event{e}{_1} and \event{e}{_2} in the minimal trace.
% \mike{Actually any contradiction will do. :)}

To help prove the theorem, we use the following lemma:

\begin{lem}
  Given a pseudo-valid trace \trPrime that has no pseudo-predictable races
  \mike{Seems weird to talk about whether \trPrime has pseudo-predictable races.
  If \tr has no pseudo-predictable races, then a pseudo-valid reordering of \tr should have no pseudo-predictable races, although we haven't established that formally.}
  and
  that is minimal with respect to the number of events between \event{e}{_1} and
  \event{e}{_2}, for any event \event{e} such that
  \TRPrimeOrdered{\event{e}{_1}}{\TRPrimeOrdered{\event{e}}{\event{e}{_2}}}, it
  is true that \DCOrdered{\event{e}{_1}}{\DCOrdered{\event{e}}{\event{e}{_2}}}.
  \mike{Do \DC and other partial orders here apply to the original trace \tr or the reordered trace \trPrime?
  (It seems like circular reasoning to me to assume that it doesn't matter.)}
%  \sout{and \nWBROrdered{\event{e}}{\event{e}{_2}}}.
  \label{lem:wbr:dc-between-e1-e2}
\end{lem}

\begin{proof}[Proof of lemma]

  We prove the lemma by contradiction.
  Let \event{e} be the \emph{first} event in \trPrime such
  \TRPrimeOrdered{\event{e}{_1}}{\TRPrimeOrdered{\event{e}}{\event{e}{_2}}} and
  \nDCOrdered{\event{e}{_1}}{\event{e}}.
  % Assume that such an event exists.
  Consider a trace \trDoublePrime that is the
  same as \trPrime except that \event{e} is ordered immediately before \event{e}{_1}.
  \trDoublePrime cannot be a pseudo-valid reordering of \tr because
  i.e., \trDoublePrime would have fewer events between \event{e}{_1} and \event{e}{_2} than \trPrime,
  violating the minimality assumption of \trPrime.
  \trDoublePrime is \emph{not} a pseudo-valid reordering because it violates
  at least one of the two rules of pseudo-valid reordering (Definition~\ref{??}):

  \subparagraph{Case 1:}
  \trDoublePrime violates the \PO rule.
  
  Then there must exist an event \event{e}{'} such that
  \EqTRPrimeOrdered{\event{e}{_1}}{\TRPrimeOrdered{\event{e}{'}}{\event{e}}} and \POOrdered{\event{e}{'}}{\event{e}}.
  Since \EqTRPrimeOrdered{\event{e}{_1}}{\TRPrimeOrdered{\event{e}{'}}{\event{e}}} and
  \event{e} is the first event such that \nDCOrdered{\event{e}{_1}}{\event{e}}, 
  therefore $\DCOrdered{\event{e}{_1}}{\event{e}{'}} \lor \event{e}{_1} = \event{e}{'}$. By Rule~(c) of
  \DC, \DCOrdered{\event{e}{'}}{\event{e}}, and using Rule~(d) we get
  \DCOrdered{\event{e}{_1}}{\event{e}}, which is a contradiction.

  \subparagraph{Case 2:}
  \trDoublePrime violates the LW rule.
  
  If \trDoublePrime violates CA,
  then there must be an event \event{e}{'} such that
  \EqWDCOrdered{\event{e}{_1}}{\event{e}{'}} and
  \conflicts{\event{e}{'}}{\event{e}}. Note that $\event{e}{_1}=\event{e}{'}$ is
  possible.
  We know that \nDCOrdered{\event{e}{'}}{\event{e}} because otherwise \DCOrdered{\event{e}{_1}}{\event{e}} by \DC Rule~(d),
  which would be a contradiction.
  Let $L=\commonLocks{\event{e}{}}{\event{e}{'}}$. If $L=\emptyset$,
  then by Theorem~\ref{thm:dc-pseudo-sound}, \tr has pseudo-predictable race,
  which is a contradiction.
  \mike{Added use of Theorem~\ref{thm:dc-pseudo-sound} here, since it seemed like we needed it. Did I miss another way you were making this argument?}
  
  Otherwise
  $L\neq\emptyset$.
  % Let $l \in L$. There must exist release events \event{r}{'}
  % and \event{r} on $l$ such that
  % \POOrdered{\event{e}{'}}{\TROrdered{\event{r}{'}}{\POOrdered{\event{e}}{\event{r}}}}.
  % Then, using \DC Rule (a) it must be that \DCOrdered{\event{r}{'}}{\event{e}}, and by \DC Rule (c)
  Then by \DC Rule~(a), we have \DCOrdered{\event{e}{'}}{\event{e}} and thus
  by \DC Rule~(d) \DCOrdered{\event{e}}{\event{e}{_1}}, which is a contradiction.

  \medskip
  \noindent
  Thus all cases lead to contradiction, so therefore
  \DCOrdered{\event{e}{_1}}{\event{e}} for any \event{e} such that
  \TRPrimeOrdered{\event{e}{_1}}{\TRPrimeOrdered{\event{e}}{\event{e}{_2}}}.

  A similar argument can be repeated for \event{e} and \event{e}{_2}, which will
  prove that \DCOrdered{\event{e}}{\event{e}{_2}}.
% %
  \kaan{This section should be expanded to show that
    \DCOrdered{\event{e}}{\event{e}{_2}}.
  \mike{Seems like we don't need that? Can we instead just narrow the lemma statement?}}
% %
\end{proof}

\noindent
With this lemma proved,
we can now prove the theorem.

% There can not be an event \event{e} such that
% \EqTRPrimeOrdered{\event{e}{_1}}{\TRPrimeOrdered{\event{e}}{\event{e}{_2}}}
% and \nPOOrdered{\event{e}}{\event{e}{_2}}.
% Assume that such an event exists. Let \event{e} be the last such event.

Let \event{e} be the last event in \trPrime such that
\EqTRPrimeOrdered{\event{e}{_1}}{\TRPrimeOrdered{\event{e}}{\event{e}{_2}}}
and \nPOOrdered{\event{e}}{\event{e}{_2}}.
(Such an event must exist because of the possibility that $\event{e} = \event{e}{_1}$.)

We consider the following exhaustive set of cases:

\subparagraph{Case 1:}
$\event{e} = \event{e}{_1}$

Then let \event{e}{'} be the event immediately following \event{e}{_1} in \trPrime
(i.e., $\TRPrimeOrdered{\event{e}{_1}}{\TRPrimeOrdered{\event{e}{'}}\event{e}{_2}} \land
\nexists \event{e}{''} \mid \TRPrimeOrdered{\event{e}{_1}}{\TRPrimeOrdered{\event{e}{''}}{\event{e}{'}}}$).
Since there is no event between \event{e}{_1} and \event{e}{_2} that is not \PO ordered to \event{e}{_2},
therefore \POOrdered{\event{e}{'}}{\event{e}{_2}}.
Reordering consecutive events \event{e}{_1} and \event{e}{'} cannot
produce a pseudo-valid reordered trace because \trPrime is a minimal trace.
Thus it must be the case that \conflicts{\event{e}{_1}}{\event{e}{'}},
% \mike{Rather than contradicting the assumption of no earlier \WBR-race,
%   doesn't this simply violate the assumption of no predictable race? Revised accordingly.
%   \kaan{Yes.}}
which implies that \tr has a predictable race, which contradicts an initial assumption.

\subparagraph{Case 2:}
$\event{e} \ne \event{e}{_1}$, and \event{e}{} is a write event

Since \trPrime is a minimal trace,
it must be the case that \event{e} cannot be moved to immediately after \event{e}{_2}
to produce a new pseudo-valid reordered trace.
By the defintion of a pseudo-valid reordered trace,
there must exist read event \event{e}{'} and branch event \event{e}{''} such that
\BrDepsOn{\event{e}{'}}{\event{e}{''}},
\TRPrimeOrdered{\event{e}}{\POOrdered{\event{e}{'}}{\POOrdered{\event{e}{''}}{\event{e}{_2}}}},
and \conflicts{\event{e}}{\event{e}{'}}.
By Rule~\ref{rel:wbr:wr-rd} of the \WBR definition,
we have \WBROrdered{\event{e}}{\event{e}{''}},
which implies \WBROrdered{\event{e}}{\event{e}{_2}}
by Rule~\ref{rel:wbr:po-right}.
By Lemma~\ref{lem:wbr:dc-between-e1-e2}, we have
\DCOrdered{\event{e}{_1}}{\event{e}}.
Finally, Rule~\ref{rel:wbr:dc-left} of \WBR
implies that \WBROrdered{\event{e}{_1}}{\event{e}{_2}},
which contradicts an initial assumption.

% Assume that \event{e} is a write. If there is no read \event{e}{'} and branch
% \event{e}{''} such that
% \TRPrimeOrdered{\event{e}}{\POOrdered{\event{e}{'}}{\POOrdered{\event{e}{''}}{\event{e}{_2}}}}
% and \conflicts{\event{e}}{\event{e}{'}}, then there exists a pseudo-valid
% reordering where \event{e} is ordered after \event{e}{_2}: such a reordering
% does not change the last writer of any read with a dependent branch. This shows
% that if $\event{e} = \event{e}{_1}$ then there exists a predictable race, or
% $\event{e} \neq \event{e}{_1}$ and this
% contradicts the definition of a minimal reordering and such an \event{e} can
% not exist. If \event{e}{'} and \event{e}{''} both do exist, then using
% Rule~\ref{rel:wbr:wr-rd} we have \WBROrdered{\event{e}}{\event{e}{''}}. Using
% Rule~\ref{rel:wbr:po-right} and Lemma~\ref{lem:wbr:dc-between-e1-e2}, we have
% \WBROrdered{\event{e}{_1}}{\event{e}{_2}}. This is a contradiction of the
% theorem statement.

\subparagraph{Case 3:}
$\event{e} \ne \event{e}{_1}$, and \event{e}{} is \emph{not} a write event

By the definition of a pseudo-valid reordered trace,
\event{e}{} can be moved after \event{e}{_2} in a pseudo-valid reordered trace,
which contradicts the assumption of a minimal trace.

% For any other \event{e}, there always exists a pseudo-valid reordering where
% \event{e} can be reordered after \event{e}{_2}. If \event{e} is a branch,
% acquire or release, then it can be reordered. Using the definition of a minimal
% reordering there can not be an event \event{e}{'} that is
% \POOrdered{\event{e}}{\event{e}{'}}, as \event{e} is the last event in its
% thread before \event{e}{_2}. Then, if \event{e} is a read there is no
% branch that depends on \event{e} in \trPrime, and there exists a pseudo-valid
% reordering where \event{e} is after \event{e}{_2}. In any of these cases, a reordering with fewer events between \event{e}{_1} and
% \event{e}{_2} exists or $\event{e} = \event{e}{_1}$ and a pseudo-predictable
% race exists, both of which are contradictions.

\medskip
\noindent
Thus all cases lead to contradiction, so \tr must have a pseudo-predictable race.
\end{proof}


==> addConstraints-CORE.tex <==
%auto-ignore
\begin{figure}
\small
\centering
\sf
\begin{tabular}{@{}lll@{}}
\textnormal{Thread 1} & \textnormal{Thread 2} & \textnormal{Thread 3}\\\hline
\Write{y}\tikzmark{4} \\
\Acquire{m}\tikzmark{10}\tikzmark{14} \\
{} \Write{z}\tikzmark{7} \\
\Release{m}\tikzmark{15} \\
					  & \tikzmark{16}\Acquire{m}\tikzmark{12} \\
					  & {} \tikzmark{8}\Read{z} \\
				 	  & {} \Write{x}\tikzmark{5} \\
					  & \Release{m}\tikzmark{1}\tikzmark{13}\tikzmark{17} \\
                      &						  & \tikzmark{18}\Acquire{m} \\
                      &						  & {} \tikzmark{6}\Read{x} \\
                      &						  & {} \tikzmark{2}\BrUniv \\
                      & 					  & \Release{m}\tikzmark{3}\tikzmark{9}\tikzmark{11} \\
                      &						  & \Read{y}
\end{tabular}
\textunderlink{1}{2}{\WBR}%
\init{3}{4}{0}{0}%
\textlink{5}{6}{\LW}%
\textlink{7}{8}{\LW}%
\back{9}{10}{30}{0}%
\back{11}{12}{30}{0}%
\back{13}{14}{30}{0}%
\link{15}{16}%
\link{17}{18}%

\jake{Maybe suppress \LS constraints and say a cycle is found after adding \LW constraints.}

\mike{Let's note in caption that this is the same execution as Figure~\ref{fig:CORE}.
\jake{Added, assuming we use Figure~\ref{fig:wr-wr-conflict:original}.
The rest of the caption needs to be changed.}}

\mike{Our two vindication examples---this figure and Figure~\ref{fig:constraints:complex-noRace}---both have no predictable race.
\jake{Right. I can use Figure~\ref{fig:wr-wr-conflict:original} instead. Same
sort of structured example, but no race with one less event.}}

\note{This figure has been removed from the paper.}

\caption{Example execution from Figure~\ref{fig:wr-wr-conflict:original} with a
\WBR-race (\ie, \nWBROrdered{\Write{y}{}}{\Read{y}{}}), but no predictable race.
Intuitively, no valid reordering exists because \Write{z} and \Read{z} must be \CORE events
(because \Write{x} and \Read{x} must be \CORE events) in any attempted valid reordering.
\label{fig:constraints:CORE}}
\end{figure}

==> complex-noRace.tex <==
%auto-ignore
\begin{figure}
\small
\centering
\sf
\begin{tabular}{@{}lllll@{}}
\textnormal{Thread 1} & \textnormal{Thread 2} & \textnormal{Thread 3} & \textnormal{Thread 4} & \textnormal{Thread 5}\\\hline
					  & \Acquire{m} \\
					  & {} \Acquire{n} \\
					  & {} \tikzmark{7}\Sync{t} \\
\Sync{t}\tikzmark{8} \\
\Acquire{p} \\
{} \textbf{\Write{x}} \\
{} \Sync{o}\tikzmark{1} \\
{} \Write{z} \\
\Release{p} \\
					  & {} {} \tikzmark{2}\Sync{o} \\
				 	  & {} \Release{n} \\
					  & \Release{m} \\
					  &						  &						  & \Acquire{n} \\
					  &						  &						  & {} \Sync{q}\tikzmark{3} \\
					  &						  &						  &						  & \tikzmark{4}\Sync{q} \\
					  &						  &						  &						  & \Acquire{p} \\
					  &						  &						  &						  & {} \Read{z} \\
					  &						  &						  &						  & \Release{p} \\
					  &						  &						  &						  & \textbf{\Read{x}} \\
					  &						  &						  &						  & \Acquire{l} \\
					  &						  &						  &						  &	{} \Write{y} \\
					  &						  &						  &						  & \Release{l} \\
                      &						  & \Acquire{m} \\
                      &						  & {} \Sync{s}\tikzmark{5} \\
                      &						  &	{} \Acquire{l} \\
                      &						  &	{} {} \Read{y} \\
                      &						  &	{} {} \BrUniv \\
                      &						  &	{} \Release{l} \\
                      & 					  & \Release{m} \\
                      &						  &						  & {} \tikzmark{6}\Sync{s} \\
					  &						  &						  & \Release{n}
\end{tabular}
\textlink{1}{2}{\WBR}%
\textlink{3}{4}{\WBR}%
\textlink{5}{6}{\WBR}%
\textlink{7}{8}{\WBR}%

\mike{Omit this figure and just show the later figure that shows two steps of \textsc{AddConstraints} adding edges?
\jake{I think that would be fine. The example is only used for this section
anyway. Should we maybe have no constraints on left and then all constraints
on right or leave the later figure as is?}}

\note{This figure has been removed from the paper.}

\caption{Example execution with a \WBR-race 
(\ie, \nWBROrdered{\Write{y}{}}{\Read{y}{}}), but no predictable race.
Intuitively, no valid reordering exists because \Write{z} and \Read{z} must be \CORE events
(because \Write{x} and \Read{x} must be \CORE events) in any attempted valid reordering.
\Sync{o} is an abbreviation for the sequence \Acquire{o}\code{;} \Read{oVar}\code{;} \BrUniv{}\code{;} \Write{oVar}\code{;} \Release{o}.}
\label{fig:complex-noRace}
\end{figure}

==> race-tables.tex <==
%auto-ignore
\centering
\small
\newcommand{\sr}[1]{#1}   % static races
\newcommand{\dr}[1]{(#1)} % dynamic races
\newcommand{\none}{\mc{1}{r@{$\;\;\textcolor{white}{\rightarrow}\;\;$}}{0}}
\newcommand{\K}[2]{#2$\;\!$K}
\newcommand{\Mm}[2]{#2$\;\!$M}

% \begin{tabular}{@{}l|rr|rr@{}}
% Program & \mc{2}{c|}{\WCP-races} & \mc{2}{c|}{\BR-races} \\
% \hline
% avrora & 5 & (202322) &5 & (204843) \\
% batik & 0 & (0) &0 & (0) \\
% h2 & 8 & (37679) &8 & (42764) \\
% luindex & 0 & (0) &1 & (1) \\
% lusearch & 0 & (0) &0 & (0) \\
% pmd & 5 & (124) &7 & (332) \\
% sunflow & 1 & (3) &2 & (8) \\
% tomcat & 80 & (23460) &92 & (24295) \\
% xalan & 15 & (352789) &47 & (1386008) \\
% \end{tabular}

% \begin{tabular}{@{}l|rr|rr@{}}
% Program & \mc{2}{c|}{\WDC-races} & \mc{2}{c|}{\WBR-races} \\
% \hline
% avrora & 3 & (202613) & 3 & (404851) \\
% batik & 0 & (0) & 0 & (0) \\
% h2 & 9 & (41627) & 9 & (46949) \\
% luindex & 1 & (1) & 1 & (1) \\
% lusearch & 0 & (0) & 1 & (6) \\
% pmd & 8 & (513) & 9 & (688) \\
% sunflow & 2 & (14) & 2 & (26) \\
% tomcat & 75 & (23169) & 314 & (86344) \\
% xalan & 20 & (293049) & 151 & (12593145) \\
% \end{tabular}

\begin{tabular}{@{}l|rr|rr||rr|rr@{}}
Program & \mc{2}{c|}{\WCP-races} & \mc{2}{c||}{\BR-races} & \mc{2}{c|}{\WDC-races} & \mc{2}{c}{\WBR-races} \\
\hline
avrora & 5 & (\K{202129}{202}) & 5 & (\K{204683}{205}) & 3 & (\K{202675}{203}) & 3 & (\K{404387}{404}) \\
batik & 0 & (0) & 0 & (0) & 0 & (0) & 0 & (0) \\
h2 & 9 & (\K{37950}{38}) & 9 & (\K{42986}{43}) & 9 & (\K{41734}{42}) & 9 & (\K{46976}{47}) \\
luindex & 0 & (0) & 1 & (1) & 1 & (1) & 1 & (1) \\
lusearch & 0 & (0) & 0 & (0) & 0 & (0) & 1 & (6) \\
pmd & 5 & (62) & 7 & (270) & 8 & (451) & 9 & (569) \\
sunflow & 1 & (5) & 2 & (9) & 2 & (14) & 2 & (24) \\
tomcat & 77 & (\K{23770}{24}) & 91 & (\K{24798}{25}) & 77 & (\K{21530}{22}) & 320 & (\K{83665}{84}) \\
xalan & 16 & (\K{353977}{354}) & 48 & (\Mm{1390644}{1.4}) & 20 & (\K{292320}{292}) & 151 & (\Mm{12584420}{13}) \\
\end{tabular}

% \mike{We can squeeze this into one column, by using the \textbackslash K macro once the results are finalized (see the use of it in Table~\ref{tab:races}).
% And/or we could just put all race results in the same row of a long table, but I guess you avoided that because it's so much data?}

\caption{Static and dynamic (in parentheses) race counts. \WCP and \BR, and \WDC
  and \WBR results are from the same set of runs.}
\label{tab:races-comparison}

% \end{table}
\smallskip
% \begin{table}[t]


==> relation-DC.tex <==
%auto-ignore
\begin{definition}[\DcFull]

% Note that Rule~\ref{dc:rule-a} and Rule~\ref{dc:rule-b} are the same as in \WCP's definition of rules with the same name.

Given a trace \tr,
\DCOrdered{}{} is the smallest relation that satisfies the following properties:

\begin{enumerate}[label=(\alph*),leftmargin=*]
  \item Same as \WCP rule~\ref{wcp:rule-a} (but for \DC instead of \WCP).
%   If two critical sections on the same lock contain \conflictingEvents,
%   then the first critical section is ordered by \DC to the second \conflictingEvent.
%   % %
%   That is, \DCOrdered{\event{r}{_1}}{\event{e}{_2}} if
%   \event{r}{_1} and \event{r}{_2} are release events on the same lock,
%   \TROrdered{\event{r}{_1}}{\event{r}{_2}},
%   $\event{e}{_1} \in \CS{\event{r}{_1}}$, $\event{e}{_2} \in \CS{\event{r}{_2}}$, and
%   \conflicts{\event{e}{_1}}{\event{e}{_2}}.
  \label{dc:rule-a}
  
  \item Same as \WCP rule~\ref{wcp:rule-b} (but for \DC instead of \WCP).
%   \item Release events on the same lock are ordered by \DC
%   if their critical sections contain \DC-ordered events.
%   Because of the next two rules, this rule can be expressed simply as follows:
%   \DCOrdered{\event{r}{_1}}{\event{r}{_2}} if
%   \event{r}{_1} and \event{r}{_2} are release events on the same lock and
%   \DCOrdered{\getAcquire{\event{r}{_1}}}{\event{r}{_2}}.
  \label{dc:rule-b}\label{wbr:rule-b}
  
  \item Two events are ordered by \DC if they are ordered by \PO.
  That is, \DCOrdered{\event{e}{}}{\event{e}{'}}
  if \POOrdered{\event{e}{}}{\event{e}{'}}. \label{dc:po}\label{wbr:po}
  
  \item \DC is transitively closed.
  That is, \DCOrdered{\event{e}{}}{\event{e}{'}} 
  if $\exists e'' \mid \DCOrdered{\event{e}{}}{\event{e}{''}} \land \DCOrdered{\event{e}{''}}{\event{e}{'}}$. \label{dc:transitive}\label{wbr:transitive}
  
\end{enumerate}
\label{def:doesnt-commute}
\end{definition}


==> relation-HB.tex <==
%auto-ignore
\begin{definition}[\HbFull] 

Given a trace \tr,
\textit{\ltHB} is the smallest relation that satisfies the following properties:

\begin{itemize}[leftmargin=*]

  \item Release and acquire events on the same lock are ordered by \HB.
  % (a.k.a.\ \emph{synchronization order}).
  That is, \HBOrdered{\event{r}{}}{\event{a}{}} if
  \event{r}{} and \event{a}{} are release and acquire events
%   respectively,
  on the same lock and \TROrdered{r}{a}. \label{hb:rel-acq}
  
  \item Two events are ordered by \HB if they are ordered by \PO.
  That is,
  \HBOrdered{e}{e'} if \POOrdered{e}{e'}. \label{hb:po}
  
  \item \HB is transitively closed. 
  That is,
  \HBOrdered{e}{e'} if $\exists e'' \mid \HBOrdered{e}{e''} \land \HBOrdered{e''}{e'}$. \label{hb:transitive}

\end{itemize} 

\label{def:happens-before}
\end{definition}


==> relation-WCP.tex <==
%auto-ignore
\begin{definition}[\WcpFull]

Given a trace \tr,
\WCPOrdered{}{} is the smallest relation that satisfies the following:

\begin{enumerate}[label=(\alph*),leftmargin=*]  
  \item If two critical sections on the same lock contain \conflictingEvents,
  then the first critical section is ordered by \WCP before the second \conflictingEvent.
  % %
  That is, \WCPOrdered{\event{r}{_1}}{\event{e}{_2}} if
  \event{r}{_1} and \event{r}{_2} are release events on the same lock,
  \TROrdered{\event{r}{_1}}{\event{r}{_2}},
  $\event{e}{_1} \in \CS{\event{r}{_1}}$, $\event{e}{_2} \in \CS{\event{r}{_2}}$, and
  \conflicts{\event{e}{_1}}{\event{e}{_2}}. \label{wcp:rule-a}
  
  \item Release events on the same lock are ordered by \WCP
  if their critical sections contain \WCP-ordered events.
  Because of the next rule, this rule can be expressed simply as follows:
  \WCPOrdered{\event{r}{_1}}{\event{r}{_2}} if
  \event{r}{_1} and \event{r}{_2} are release events on the same lock and
  \WCPOrdered{\getAcquire{\event{r}{_1}}}{\event{r}{_2}}. \label{wcp:rule-b}\label{br:rule-b}

  \item \WCP is closed under composition with \HB.
  That is, \WCPOrdered{e}{e'} 
  if $\exists e'' \mid \WCPOrdered{\HBOrdered{e}{e''}}{e'} \lor
                       \HBOrdered{\WCPOrdered{e}{e''}}{e'}$. \label{wcp:hb-composition}\label{br:hb-comp}
\end{enumerate}
\label{def:weak-causally-precedes}
\end{definition}


==> vindication-tables.tex <==
%auto-ignore
\centering
\small
% \newcommand{\sr}[1]{#1}   % static races
% \newcommand{\dr}[1]{(#1)} % dynamic races
\newcommand{\none}{\mc{1}{r@{$\;\;\textcolor{white}{\rightarrow}\;\;$}}{0}}
\newcommand{\K}[2]{#2$\;\!$K}

\begin{tabular}{@{}l|rr|rr|r@{$\;\;\rightarrow\;\;$}l@{}}
Program & \mc{2}{c|}{\BR-races} & \mc{2}{c|}{\WBR-races} & Pot. & Ver. \\
\hline
\bench{avrora} & 5 & (\K{202,719}{203}) &5 & (\K{406,096}{406}) & \none \\
\bench{batik} & 0 & (0) &0 & (0) & \none \\
\bench{h2} & 11 & (\K{43,355}{43}) &11 & (\K{47,200}{47}) & 1 & 0 \\
\bench{luindex} & 1 & (1) &1 & (1) & \none \\
\bench{lusearch} & 0 & (0) &1 & (6) & 1 & 0 \\
\bench{pmd} & 5 & (42) &9 & (510) & 5 & 5 \\
\bench{sunflow} & 2 & (9) &2 & (24) & \none \\
\bench{tomcat} & 99 & (\K{25,782}{26}) &322 & (\K{81,185}{81}) & 223 & 47 \\
\bench{xalan} & 31 & (\K{1,068,577}{1,069}) &157 & (\K{12,540,837}{12,541}) & 126 & 126 \\
\end{tabular}
\caption{Static and dynamic (in parentheses) race counts.
The \colname{Pot. $\rightarrow$ Ver.} column reports static \WBR-only races,
followed by how many static \WBR-only races were verified as predictable races by \checkWBRRace.
The static race counts are not comparable to Table~\ref{tab:races-comparison} due to differences in static race counting.}
\label{tab:races}
\smallskip


\caption{Characteristics of the distribution of event distances of \WBR-only races that are true predictable races.}
\label{tab:race-distances}

